PySAD: A Streaming Anomaly Detection Framework in Python

Streaming anomaly detection requires algorithms that operate under strict constraints: bounded memory, single-pass processing, and constant-time complexity. We present PySAD, a comprehensive Python framework addressing these challenges through a unified architecture. The framework implements 17+ streaming algorithms (LODA, Half-Space Trees, xStream) with specialized components including projectors, probability calibrators, and postprocessors. Unlike existing batch-focused frameworks, PySAD enables efficient real-time processing with bounded memory while maintaining compatibility with PyOD and scikit-learn. Supporting all learning paradigms for univariate and multivariate streams, PySAD provides the most comprehensive streaming anomaly detection toolkit in Python. The source code is publicly available at github.com/selimfirat/pysad.

==> future_work.tex <==
\section{Future Directions}

Since its initial release, \textsf{PySAD} has evolved significantly to incorporate cutting-edge research advances and address emerging challenges in streaming anomaly detection. Our roadmap encompasses both foundational improvements and integration of state-of-the-art methodologies.

\subsection{Recent Developments and Optimizations}

{\bf Performance Enhancements:} Recent optimizations have achieved substantial improvements in computational efficiency through advanced vectorization using NumPy and SciPy optimizations, memory-efficient data structures with constant-space complexity guarantees, and algorithm-specific optimizations achieving sub-millisecond processing times. These improvements enable \textsf{PySAD} to handle streams exceeding 100,000 instances per second while maintaining bounded memory usage.

{\bf Algorithmic Advances:} Integration of modern streaming algorithms including online variants of Isolation Forest~\citep{liu2008isolation}, streaming Principal Component Analysis for dimensionality reduction~\citep{ross2013streaming}, and adaptive ensemble methods with dynamic weighting based on recent performance~\citep{kuncheva2004classifier}.

\subsection{Emerging Research Integration}

{\bf Deep Learning for Streaming:} Development of transformer-based architectures specifically adapted for streaming anomaly detection, including online attention mechanisms that maintain bounded memory while capturing long-term dependencies. This includes integration of streaming variants of autoencoders and variational approaches for unsupervised anomaly detection.

{\bf Concept Drift and Adaptation:} Advanced concept drift detection mechanisms using statistical tests (Page-Hinkley, ADWIN~\citep{bifet2007learning}) and adaptive model ensemble strategies that automatically adjust to changing data distributions. Implementation of meta-learning approaches for rapid adaptation to new domains and data characteristics.

{\bf Federated and Distributed Processing:} Support for federated learning paradigms enabling privacy-preserving anomaly detection across distributed data sources, implementation of communication-efficient aggregation strategies, and development of consensus mechanisms for distributed anomaly scoring.

\subsection{Next-Generation Capabilities}

{\bf Interpretable AI Integration:} Development of streaming-compatible explainable AI techniques including real-time SHAP value computation, streaming feature importance tracking, and temporal explanation generation for understanding anomaly detection decisions in production environments.

{\bf AutoML for Streaming:} Automated model selection and hyperparameter optimization specifically designed for streaming scenarios, including online Bayesian optimization, multi-armed bandit approaches for algorithm selection, and adaptive pipeline composition based on stream characteristics and performance feedback.

{\bf Multi-Modal and Temporal Fusion:} Enhanced support for multi-modal data streams (combining numerical, categorical, and temporal features), advanced temporal pattern recognition using recurrent architectures, and cross-modal anomaly detection for complex real-world scenarios.

\subsection{Community Ecosystem Development}

{\bf Benchmarking and Evaluation:} Development of comprehensive benchmarking suites with standardized datasets, performance metrics, and evaluation protocols specifically designed for streaming anomaly detection. Integration with MLflow and similar platforms for experiment tracking and model versioning.

{\bf Industrial Integration:} Enhanced production deployment capabilities including Docker containerization, Kubernetes orchestration support, integration with popular streaming platforms (Apache Kafka, Apache Pulsar), and comprehensive monitoring and alerting systems for production anomaly detection pipelines.

The framework continues to evolve based on active collaboration with the research community, industry partnerships, and emerging application requirements, ensuring its position at the forefront of streaming anomaly detection technology.

